Learning Abstractions for Program Synthesis

Many example-guided program synthesis techniques use abstractions to prune the search space. While abstraction-based synthesis has proven to be very powerful, a domain expert needs to provide a suitable abstract domain, together with the abstract transformers of each DSL construct. However, coming up with useful abstractions can be non-trivial, as it requires both domain expertise and knowledge about the synthesizer. In this paper, we propose a new technique for learning abstractions that are useful for instantiating a general synthesis framework in a new domain. Given a DSL and a small set of training problems, our method uses tree interpolation to infer reusable predicate templates that speed up synthesis in a given domain. Our method also learns suitable abstract transformers by solving a certain kind of second-order constraint solving problem in a data-driven way. We have implemented the proposed method in a tool called ATLAS and evaluate it in the context of the BLAZE meta-synthesizer. Our evaluation shows that (a) ATLAS can learn useful abstract domains and transformers from few training problems, and (b) the abstractions learned by ATLAS allow BLAZE to achieve significantly better results compared to manually-crafted abstractions.

==> impl.tex <==
\section{Implemention and Instantiations}

We have implemented the \atlas algorithms in a tool, written in Java, which takes as input a DSL (with axiomatic semantics of the DSL constructs) and a set of synthesis problems, and has access to an Abstraction-Guided Synthesizer. We have instantiated \atlas for two application domains, string transformation and matrix manipulation. In what follows, we describe our implementation of \atlas and its instantiations. 

\paragraph{Implementation.} 
Our implementation consists of two main procedures, namely \textsc{LearnAbstractDomain} and \textsc{LearnTransformers}. 
In particular, we use iZ3 which is a built-in function in the Z3 theorem prover~\cite{z3} to compute the tree interpolant in the \textsc{LearnAbstractDomain} procedure. \todo{Greg: Please explain how to implement the Solve function \textsc{LearnTransformers}, e.g., what library is used.}




==> intro-old.tex <==
\section{Introduction} 


Program synthesis is a powerful technique for automatically generating programs from high-level specifications, such as input-output examples. Due to its myriad use cases across a wide range of application domains (e.g., spreadsheet automation~\cite{flashfill,singh2016}, data science~\cite{morpheus,dace}, cryptography~\cite{synudic,dual}, improving programming productivity~\cite{sypet,insynth,prospector}, ...), program synthesis has received widespread attention from the research community in recent years.

Because program synthesis is -- in essense -- a very difficult search problem, many recent solutions  prune the search space by utilizing \emph{program abstractions}~\cite{lambda2,morpheus,synquid,blaze}.  For example, state-of-the-art synthesis tools, such as \blaze~\cite{blaze}, \morpheus~\cite{morpheus}, Scythe~\cite{scythe} and \textsc{Simpl}~\cite{So2017}, symbolically execute (partial) programs over some abstract domain and reject those programs whose abstract behavior is inconsistent with the specification. Because many programs share the same  behavior in terms of their abstract semantics, the use of abstractions allows these synthesis tools to significantly reduce the search space. 


While abstraction-guided synthesis has proven to be quite powerful, these techniques require a domain expert to manually come up with a suitable abstract domain and write abstract transformers for each DSL construct. For instance, while \blaze is a general-purpose synthesis framework that can be used in any application domain, an expert needs to manually specify a universe of predicate templates, together with sound abstract transformers  for every DSL construct. As another example, \morpheus also requires an abstract domain in the form predicate templates as well as the abstract semantics of every library method that can be used by the synthesizer.
Unfortunately, this process is not only time-consuming but also requires significant insight about the application domain as well as the internal workings of the synthesizer. 


In this paper, we propose a novel technique for automatically learning  domain-specific abstractions  that are useful for instantiating a general-purpose synthesis framework in a new domain. Given a new DSL and a training set of synthesis problems, our method learns  a useful abstract domain (in the form of predicate templates) as well as abstract transformers for each DSL construct. In addition to eliminating the significant manual effort required from a domain expert, the abstractions learned by our method often outperform manually-crafted ones in terms of their benefit to synthesizer performance.





The workflow of our approach, henceforth called \atlas~\footnote{\atlas stands for \underline{A}u\underline{T}omated \underline{L}earning of \underline{A}b\underline{S}tractions.}, is shown schematically in \figref{workflow}. Since \atlas is meant to be used as an \emph{off-line} training step for a general-purpose (abstraction-guided) synthesizer, it takes as input a new DSL as well as a set of synthesis problems (i.e., specifications) $\vec{\spec}$ that can be used for training purposes. Given these inputs, our method enters a refinement loop where an \emph{Abstraction Learner (AL)} component poses a sequence of increasingly more difficult synthesis problems $\vec{\psi}_1, \ldots, \vec{\psi}_n$ to a \emph{Generic Synthesizer (GS)}, which is in turn guided by a sequence of more precise abstractions $\abs_1, \ldots, \abs_n$ generated by the AL. In each iteration, the Abstraction Learner uses GS  to synthesize a set of programs satisfying  $\vec{\psi}_i$ using the current abstraction $\abs_i$ and its corresponding abstract transformers $\trans_{\abs_i}$. %abstract transformers $\trans_\abs^i$ of the DSL constructs.
While the programs returned by GS are guaranteed to satisfy $\vec{\psi}_i$, they may not satisfy the actual specification $\vec{\spec}$.  The Abstraction Learner then uses this information to learn a better abstraction $\abs_{i+1}$ as well as a new set of sound abstract transformers $\trans_{\abs_{i+1}}$.  Upon termination of the algorithm, we have $\vec{\psi}_n = \vec{\spec}$, which indicates that the final abstraction $\abs_n$ and transformers $\trans_{\abs_n}$ are precise enough for solving the provided training problems. Furthermore, because our method learns \emph{general} abstractions in the form of predicate templates, the learnt transformers are expected to be useful for solving many other synthesis problems beyond those in the training set.

\begin{comment}

\todo{
The workflow of our approach, henceforth called \atlas~\footnote{\atlas stands for \underline{A}u\underline{T}omated \underline{L}earning of \underline{A}b\underline{S}tractions.}, is shown schematically in \figref{workflow}. Since \atlas is meant to be used as an \emph{off-line} training step for a general-purpose (abstraction-guided) synthesizer, it takes as input a new DSL as well as a set of synthesis tasks (i.e., specifications) $\vec{\spec}$ that can be used for training purposes. Given these inputs, our method enters a refinement loop where an \emph{Abstraction Learner (AL)} component poses a sequence of increasingly more difficult synthesis problems to a \emph{Generic Synthesizer (GS)} by over-approximating the specifications $\vec{\spec}$ using a sequence of progressively more precise abstractions $\vec{\abs}$. 
In the $i$-th iteration with specifications $\vec{\spec}^{\star}_i$ that over-approximates $\vec{\spec}$, AL uses GS to synthesize a set of programs satisfying $\vec{\spec}^{\star}_i$ using abstract transformers $\trans_{\vec{\abs}_i}$ of the DSL constructs. While the programs returned by GS in the $i$-th iteration are guaranteed to satisfy $\vec{\spec}^{\star}_i$, they may not satisfy the actual specification $\vec{\spec}$.  AL then uses this information to learn a better abstraction $\vec{\abs}_{i+1}$ as well as a new set of sound abstract transformers $\trans_{\vec{\abs}_{i+1}}$ in the next iteration. 
}
end{comment}






\begin{comment}
Our method requires two inputs, namely a DSL (including its context-free grammar and semantics) as well as training data in the form of input-output examples. Given these inputs, \atlas performs a \todo{fixed-point: why is it a fixed-point computation?} computation in which it iteratively discovers new predicate templates that are useful for synthesis, together with the corresponding abstract transformers of each DSL construct. When this fixed-point computation terminates, the generic synthesis framework is guaranteed to succeed on the provided training data using the abstractions learned by \atlas. 

\todo{(I am proposing something like the following)} 
The workflow of our approach, henceforth called \atlas~\footnote{\atlas stands for \underline{A}u\underline{T}omated \underline{L}earning of \underline{A}b\underline{S}tractions.}, is shown schematically in \figref{workflow}. Our method requires two inputs, namely a DSL (including its context-free grammar and semantics) as well as training data in the form of input-output examples $\vec{\examples_t}$. Given these inputs, \atlas iteratively discovers new predicate templates that are useful for synthesis, together with the corresponding abstract transformers of each DSL construct, until it successfully synthesizes correct programs for all training examples $\vec{\examples_t}$ with the learnt abstractions. 
\end{comment}


\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.37]{figs/workflow4.pdf}
\end{center}
\caption{Schematic overview of our approach.}
\figlabel{workflow}
\end{figure}


\begin{comment}
In more detail, \atlas works as follows: Starting with a trivial abstraction (i.e., $\top$), \atlas invokes the synthesizer to find programs $\vec{P}$ that satisfies the training examples $\vec{\examples_t}$ under this abstraction. If the synthesized programs are indeed consistent with $\vec{\examples_t}$ according to the concrete semantics, ATLAS returns the current abstraction as the result. Otherwise, it infers new predicate templates, together with their corresponding abstract transformers, and invokes the synthesizer using this new, more precise abstraction. This interaction between the Abstraction Learner and the Generic Synthesis Framework continues until the generic synthesizer is able to find the desired programs for all training examples using the current abstraction.
\end{comment}


From a technical perspective, the Abstraction Learner uses two key ideas, namely \emph{tree interpolation} and \emph{data-driven abduction}, for learning useful abstract domains and  transformers respectively. To see how these ideas are useful, consider the specifications $\vec{\spec_i}$ and abstraction $\abs_i$ that are provided to the Synthesizer during the $i$'th iteration of the algorithm. While the programs $\vec{\prog}_i$ returned by the Synthesizer are guaranteed to satisfy $\vec{\spec_i}$, they may not satisfy the stronger (but desired) specification $\vec{\spec}$. Given such a program $\prog_{ij}$ that does not satisfy the intended $\spec_j$, our method constructs a proof -- in the form of a tree interpolant -- that $\prog_{ij}$ does not satisfy $\spec_j$ and extracts new predicate templates from the formulas used in the interpolant.  Since these predicates are useful for refuting the correctness of program $\prog_{ij}$, they are used to enrich the existing abstraction through the addition of new predicate templates.

While tree interpolation is useful for learning a new abstraction $\abs$, the synthesizer ultimately needs abstract transformers over $\abs$ for each DSL construct. We formulate the problem of learning abstract transformers over $\abs$ in terms of \emph{abductive reasoning} and provide a new data-driven, counterexample-guided algorithm for solving the underlying abductive inference problem.



%there are two key innovations that allow \atlas to find abstractions that are useful for synthesis. First, \atlas automatically infers useful predicates by solving a tree interpolation problem on the incorrect programs returned by the generic synthesizer. The predicates used in the interpolants are abstracted as templates and added to the abstraction. Second, given a set of predicate templates, \atlas learns sound abstract transformers by solving an abductive reasoning problem. However, since the generated abduction problems are typically in complex theories that do not admit quantifier elimination, \atlas uses a new abductive reasoning technique based on counterexample-guided inductive synthesis. 

We have implemented these ideas in a tool called \atlas and evaluate it in the context of the \blaze program synthesis framework~\cite{blaze}.  Our evaluation shows that  the proposed technique completely eliminates the manual effort involved in designing useful abstractions and  abstract transformers. More surprisingly, our evaluation also shows that the abstractions and transformers generated automatically by \atlas outperform manually crafted ones in terms of the performance of the \blaze synthesizer in two different application domains. % namely string and matrix transformations.


%We have combined this proposed approach with a state-of-the-art abstraction-based synthesizer \blaze to learn useful domain-specific abstractions, and experimentally evaluate \blaze-\atlas in two canonical domains (i.e., string and matrix transformations) by comparing it against \blaze-manual, which is an instantiation of \blaze using manually constructed abstractions. Our experimental results show that \blaze-\atlas is more efficient compared to \blaze-manual, while requiring way less manual effort.




==> proofs.tex <==
\section{Proofs}
\label{app:proofs}

\paragraph{Proof of Theorem~\ref{thm:trans-sound}}
Note that in line 8 of \figref{learntransformer} we check the validity of the
formula $\Lambda[\vec{f}_j]$. This is the formula from
\eqnref{abduction} with $P$ replaced by $\vec{f}_j$. Note that this
formula already expresses the soundness of the transformer, so if this formula
is valid then $\tau$ is trivially sound.

\paragraph{Proof of Theorem~\ref{thm:trans-complete}}
In order to analyze the $\Call{LearnTransformers}{}$ algorithm, we need to be
formal about what we mean when we randomly sample values in line 6 of the
$\Call{GenerateExamples}{}$ algorithm. In particular, the domain of $F$ may be
infinite, in which case we must choose some finite subset of the domain to
sample. We define the example set $E$ in terms of two matrices $A,B$ such that
if $P$ is the desired transformer, then $AP=B$. Here each row of $A$ represents
in input and the corresponding row of $B$ represents the output.
Note that in order for the example input matrix $A$ to be full-rank, we need
$|\cin|+1$ linearly independent examples. By assumption, there exists a complete
sampling oracle $R_F$. Since $R_F$ has a finite support $S$, in the worst case
we can choose every example from $S$, which is sufficient to guarantee that $A$
is full-rank. Then because $A$ is full-rank, there exists a unique $P$ such that
$AP=B$.

By assumption, there exists a unique best abstract transformer $\tau$ for each
DSL operator and set of input templates $\chi_1,\ldots,\chi_n$. For each
$(\chi,\vec{f})\in\textsc{Outputs}(\tau)$, we have that $\vec{f}$ is the unique
best function for the output template $\chi$. Let $E$ be the set of examples
generated by \Call{GenerateExamples}{} for the output template $\chi$. Suppose
there we fail to learn an affine function for this set of examples. Then because
we learn this function by solving a system of linear equations, this implies
there does not exist an affine function which is consistent with all of the
examples in $E$. In this case either there does not exist an affine function
which yields a sound transformer or there exist multiple affine functions which
yield sound transformers. In the former case, there clearly cannot be a unique
best function for $\chi$ so $\tau$ cannot be a unique best abstract transformer.
In the latter case, we know $\vec{f}$ must be the unique best function for
$\chi$. But then at least one example must be consistent with some affine
function $\vec{f}'$ with $\vec{f}' \neq \vec{f}$.

Because $\vec{f}$ is the unique best function, we know that $\chi(y, \vec{f})
\Rightarrow \chi(y, \vec{f}')$. But by assumption, the \textsf{Abstract}
procedure returns the strongest abstraction for the given concrete value.
Then because $\chi(y, \vec{f}')$ is the output of the \textsf{Abstract}
procedure, we have $\chi(y, \vec{f}') \Rightarrow \chi(y, \vec{f})$  for all
$y$ so we know $\vec{f}' = \vec{f}$. Thus $(\chi, \vec{f})$ must be included in
the transformer returned by \Call{LearnTransformers}{}. Therefore the
learned transformer is at least as strong as $\tau$. But then by assumption
$\tau$ is the strongest transformer, so we must have that the learned
transformer is $\tau$.


\begin{lemma}[Progress of \textnormal{\textsc{LearnAbstractions}}]
\label{thm:abs-progress}
Let $\prog_j$ be a spurious program returned by \textnormal{\textsf{Synthesize}} in the \emph{j}'th iteration for problem $\examples_i$ in \textsc{LearnAbstractions}. 
Then, in the \emph{(j+1)}'th iteration for problem $\examples_i$, we have $\prog_{j+1} \neq \prog_j$. 
\end{lemma}

\paragraph{Proof of Lemma~\ref{thm:abs-progress}}
Because $\prog_j$ does not solve the training problem $\examples_i$ under 
concrete
semantics, there exists an input/output example $(\inex, \outex)$ such that
$\semantics{\prog_j}\inex \neq \outex$. Let $(\abs',\trans')$ be the abstract 
domain and transformers for the \emph{(j+1)}th iteration. Then following 
\figref{learndomain} we
construct an interpolation problem $T$ and find an interpolant $\itp$ for this
problem. Note that this interpolant establishes the spuriousness of $\prog_j$.
Therefore if each predicate in $\itp$ can be represented in $\abs'$ and if the
transformers in $\trans'$ are precise enough, $\prog_j$ will fail under the
abstraction $(\abs',\trans')$. Now note that the predicate templates in $\abs'$
include each predicate that appears in $\itp$ with the variables and constants
replaced by holes. Therefore each predicate in $\itp$ must be representable
in $\abs'$. By Theorem~\ref{thm:trans-complete}, we know that as long as a
transformer exists and is affine,
$\Call{LearnTransformers}{}$ will learn the strongest sound transformer. By the 
definition of an interpolant, the predicate
for each argument value conjoined with the specification of a DSL operator
implies the predicate for the output value. Therefore a transformer exists
whenever these predicates appear in the interpolant. Whenever these transformers
are affine, we can learn them. Then the program $\prog_j$ will fail on on the
example $\examples_i$ under the abstraction $(\abs',\trans')$.

\paragraph{Proof of Theorem~\ref{thm:termination}}
We assume the AGS has a deterministic ranking for programs, i.e., there exists a
bijection $f:P \to \mathbb{N}$ from the set of programs to natural numbers such
that if the AGS returns a program $\prog_1$ then for any other program $\prog_2$
which satisfies the example $\examples_i$ under the current abstraction,
$f(\prog_1) < f(\prog_2)$. Then by assumption, for
each training example $\examples_i \in \vec{\examples}$ there exists a program
$\prog$ such that $\prog$ satisfies $\examples_i$ under the concrete semantics.
There are a finite number of programs $\prog'$ for which $f(\prog') < f(\prog)$.
Let $(\abs_i, \trans_i)$ be the abstract domain and transformers for the $i$'th
iteration of the top level algorithm. Let $\prog_i$ be the program learned by
the AGS under the abstraction $(\abs_i, \trans_i)$. If $\prog_i$ does not
satisfy the current training example under concrete semantics, then by
Lemma~\ref{thm:abs-progress} $\prog_i$ is ruled out by the abstraction
$(\abs_{i+1}, \trans_{i+1})$. In particular, this means that for each $i$,
$f(\prog_{i+1}) > f(\prog_i)$. Because there are a finite number of programs
explored before $\prog$, by induction we have that eventually we will learn the
program $\prog$ (or some other program $\prog'$ which satisfies $\examples_i$
under the concrete semantics with $f(\prog')<f(\prog)$). Since we will
eventually learn the correct program for each training example,
\Call{LearnAbstractions}{} terminates.




==> transformerLearner.tex <==
\newcommand{\rank}{\ensuremath{\operatorname{rank}}}
\newcommand{\Null}{\ensuremath{\operatorname{Null}}}

%\section{Learning Transformers}
(Notation: We use $M_{m\times n}(R)$ to denote the set of $m\times n$ matrices
with entries from the ring $R$. We abbreviate $M_{n\times n}(R)$ as $M_n(R)$.
For a matrix $A$, the notation $\Null(A)$ is used to denote the null space of
$A$.)

(Aside: We are interested in programs with integer coefficients, but most
results in linear algebra require a (skew) field of scalars. Therefore we will
define all intermediate results over $\mathbb{Q}$. Aside from the final result,
this is fine because all of the computations we need to do admit scalar
multiples. Therefore we will simply cancel denominators when integers are
necessary.)

We represent our input/output examples as a matrix $X$ of inputs and a vector
$y$ of outputs, such that each row of $X$ and the corresponding element of $y$
constitute one example. That is, $(X_{i1},X_{i2},\cdots,X_{in})\mapsto  y_i$ is
an input/output example for each $i$. Then the abstract transformer is
represented by a vector $p$ such that $Xp=y$.

Suppose we have an oracle which can give us the expected output for a given set
of inputs. Then we let the input matrix $X\in M_{n}(\mathbb{Q})$ be defined as
\[X=\begin{bmatrix} n & 1 & \cdots & 1 \\
  1 & n & \cdots & 1 \\
\vdots & \vdots & \ddots & \vdots \\
1 & 1 & \cdots & n \end{bmatrix}\]
That is, the diagonal elements of $X$ are $n$, and all other elements are 1.
Then we compute the output vector $y$ such that $X$ and $y$ satisfy the
assumptions on input/outputs examples.

Note that $\rank(X)=n$ which can be shown as follows: let $0\neq
a\in\mathbb{Q}$. Then there exists some $M$ with $1\le M\le n$ such that
$|a_M|\ge |a_i|$ for all $1\le i\le n$ Since $a\neq 0$, we have $|a_M|>0$. Now
let $b=Xa$. Then
\[b_M=\sum_{i=1}^nX_{Mi}a_i=X_{MM}a_M+\sum_{\substack{1\le i\le n \\ i\neq M}}
X_{Mi}{a_i}\]
and $X_{MM}=n$ and $X_{Mi}=1$ for $i\neq M$. Then note that
\[\left|\sum_{\substack{1\le i\le n \\ i\neq M}}X_{Mi}a_i\right|\le
(n-1)\max_{\substack{1\le i\le n \\ i\neq M}}|a_i|\le (n-1)|a_M|\]
Then $|b_M|\ge n|a_M|-(n-1)|a_M|=|a_M|>0$ so $b\neq 0$. Therefore the $Xa=0\iff
a=0$ and $X$ must be full rank.

Since $X$ is known to be full-rank, there will be exactly one solution to the
system of equations $Xp=y$ over the rationals. If $p$ has only integer
coefficients then it must be the unique transformer consistent with the
given examples which can be represented in LIA. If $p$ has non-integer entries
then no such transformer exists.


